Formalising Confluence in PVS

Confluence is a critical property of computational systems which is related with determinism and non ambiguity and thus with other relevant computational attributes of functional specifications and rewriting system as termination and completion. Several criteria have been explored that guarantee confluence and their formalisations provide further interesting information. This work discusses topics and presents personal positions and views related with the formalisation of confluence properties in the Prototype Verification System PVS developed at our research group.

==> eptcsdata.tex <==
\providecommand{\firstpage}{11}
\providecommand{\publicationstatus}{C.A. Mu\~noz and J. A. P\'erez (Eds.) :\\
Developments in Computational Models\\
EPTCS 204, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.204.2}{10.4204/EPTCS.204.2}}

